Adaptive Cruise Control in Autonomous Vehicles: Challenges, Gaps, Comprehensive Review, and, Future Directions

The development of Autonomous Vehicles (AVs) has redefined the way of transportation by eliminating the need for human intervention in driving. This revolution is fueled by rapid advancements in adaptive cruise control (ACC), which make AVs capable of interpreting their surroundings and responding intelligently. While AVs offer significant advantages, such as enhanced safety and improved traffic efficiency, they also face several challenges that need to be addressed. Existing survey papers often lack a comprehensive analysis of these challenges and their potential solutions. Our paper stands out by meticulously identifying these gaps in current ACC research and offering impactful future directions to guide researchers in designing next-generation ACC systems. Our survey provides a detailed and systematic review, addressing the limitations of previous studies and proposing innovative approaches to achieve sustainable and fault-resilient urban transportation.

==> includes/tables/tabSummaryReview.tex <==
\begin{table*}[!hbp]
	\centering
	\caption{Comparison of Different EV ... Techniques}
	%\ra{1.8}
	\label{tab:prosCons}
	\begin{tabular}{@{}
			P{0.1\textwidth}
			m{0.07\textwidth}
			m{0.23\textwidth}
			m{0.23\textwidth}
			m{0.23\textwidth}
		}
		\hline
		\multicolumn{1}{c}{\textbf{Category}} &
		\multicolumn{1}{c}{\textbf{Approach}} &
		\multicolumn{1}{c}{\textbf{Advantages}} & \multicolumn{1}{c}{\textbf{Disadvantages}} &
		\multicolumn{1}{c}{\textbf{Challenges}}\\ 
		\toprule 
		
		\multirow{4}{*}{\specialcell{... \\ based}} &
		
		... based  & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} \\
		
		& ... based & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} \\
			
		\hline
		
		\multirow{4}{*}{\specialcell{... \\ based}} &
		
		... based  & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} \\
		
		& ... based & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} & 
		\begin{itemize}
			\item .
			\item .
		\end{itemize} \\
		
		\toprule
	\end{tabular}
\end{table*}
